Fast Navigation with Icosahedral Golden Gates

An algorithm of Ross and Selinger for the factorization of diagonal elements of PU(2) to within distance $\varepsilon$ was adapted by Parzanchevski and Sarnak into an efficient probabilistic algorithm for any element of PU(2) using at most effective $3\log_p\frac{1}{\varepsilon^{3}}$ factors from certain well-chosen sets associated to a number field and a prime $p$. The icosahedral super golden gates are one such set associated to $\mathbb{Q}(\sqrt{5})$. We leverage recent work of Carvalho Pinto, Petit, and Stier to reduce this bound to $\frac{7}{3}\log_{59}\frac{1}{\varepsilon^3}$, and we implement the algorithm in Python. This represents an improvement by a multiplicative factor of $\log_259\approx5.9$ over the analogous result for the Clifford+$T$ gates. This is of interest because the icosahedral gates have shortest factorization lengths among all super golden gates.

==> AlgSis.tex <==
\subsection{Diagonal elements}
\zack{need to write}
\subsection{Generic elements}
Here we largely adopt the structure and wording from \cite[\S5]{Stier}, as the core heuristics are the same as in the icosahedral setting. 

We begin the analysis by establishing the $\tau$-count and tightness of the approximation. In particular, $d(\g_1,\gd_1)<\eps$ and $d(\g_2,\gd_2)<\eps$ with factorization lengths of $\g_\ell$ each up to $(1+o(1))\log_{59}(\nicefrac{1}{\eps^3})$. By \lemref{lem:old lem}, $d(\g,\gd_1\g\gd_2)<C\eps$. Therefore, $d(g,\g_1\g\g_2)<(C+2)\eps$ (by the triangle inequality) and since $\g$ has a factorization of $\tau$-count up to $\lpr{\frac{1}{3}+o(1)}\log_{59}(\nicefrac{1}{\eps^3})$, this constitutes a factorization of an element in $g$'s neighborhood of $\tau$-count up to $\lpr{\frac{7}{3}+o(1)}\log_{59}(\nicefrac{1}{\eps^3})$. 

The efficiency of this algorithm---that is, that it runs in time $O(\poly\log(\nicefrac{1}{\eps}))$---is because we expect to halt when $59^k\eps^3\in O(1)$ (so only $k\approx\frac{1}{3}\log_{59}(\nicefrac{1}{\eps^3})$ calls are expected \zack{oops! this isn't implied...instead, something to do with because the diagonals on either side can basically be anything, so we get 2 extra degrees of freedom, which knocks down the power of $\eps$ from 3 to 1? double check with Peter to refresh the exact reasoning...}), and only call polynomially-many polynomial-time subroutines. The dominant subroutines are calls to Lenstra's algorithm which as shown in \cite{Lenstra} runs in time polynomial in the side of the constraints for any fixed dimension $n$. Indeed, here we have only $n=2$ dimensions, $m=6$ linear constraints (two per absolute value), and the largest value $a$ in the constraints is $p^k$, so the runtime is polynomial in $nm\log a\in \theta(k)$. 

The reason we expect to halt when $59^k\eps\in O(1)$ is that \zack{see issue above}

When attempting to write elements of $\cO$ as a sum of two squares, we primarily rest on a belief, in the style of Cram\'er's conjecture and a conjecture of Sardari \cite[($*$)]{Sardari} that sums of squares are dense in $\N$. Seeking to analogize \cite[($*$)]{Sardari} in particular, we note that the operative aspect is that a dense cluster of lattice points will represent at least one sum of two squares, and that such a point this will be found quickly through Lenstra's algorithm. 

The significance of this result is to accomplish a factorization in $\PU(2)$ in analogue to \cite{Stier}, but using a gate set with additional desirable properties beyond those enjoyed by the Clifford+$T$ gates. 

==> nearbyelementspu2.tex <==
For $\alpha,\beta\in\mathbb{C}$ satisfying $\abs{\alpha}^2+\abs{\beta}^2=1,$ we introduce the following notation for canonical unitary matrices 
$$u(\alpha,\beta)=\begin{pmatrix}\alpha & \beta \\ -\bar{\beta} & \bar{\alpha}\end{pmatrix}$$ and 
for $\theta\in\mathbb{R}$, we write,
$$u(\theta)=u(e^{i\theta},0)=\begin{pmatrix}e^{i\theta} \\ & e^{-i\theta}\end{pmatrix}.$$

We restate below \cite[Lemma 5]{Stier} which holds independent of our choice of universal gate set. 
\begin{lemma}\label{lem:old lem}
    Select absolute constants $\delta,\varepsilon_0>0$ and put $C=\sqrt{\half+\half\left(\frac{2+\delta}{\varepsilon_0}\right)^2}$. Take $\gamma_1$ and $\gamma_2$ in either {\em SU(2)} or {\em PU(2)} and write them as $\gamma_1(\alpha_1,\beta_1)$ and $\gamma_2=u(\alpha_2,\beta_2)$. If $\abs{\abs{\alpha_1}-\abs{\alpha_2}}<\varepsilon$ for some $\epsilon<\delta$ and $\min\{\abs{\alpha_1},\abs{\alpha_2}\}<\sqrt{1-\varepsilon_0^2}$ then for 
    \begin{align*}
        \theta_1&=\frac{1}{2}(\arg\alpha_1-\arg\alpha_2+\arg\beta_1-\arg\beta_2), & \delta_1&=u(\theta_1)\\
        \theta_2&=\frac{1}{2}(\arg\alpha_1-\arg\alpha_2-\arg\beta_1+\arg\beta_2), & \delta_2&=u(\theta_2)
    \end{align*}
    we have the approximation $\delta_1\gamma_2\delta_2$ to $\gamma_1$, satisfying
    $$d(\gamma_1,\delta_1\gamma_2\delta_2)<C\varepsilon.$$
\end{lemma}
